Single View Metrology in the Wild

Most 3D reconstruction methods may only recover scene properties up to a global scale ambiguity. We present a novel approach to single view metrology that can recover the absolute scale of a scene represented by 3D heights of objects or camera height above the ground as well as camera parameters of orientation and field of view, using just a monocular image acquired in unconstrained condition. Our method relies on data-driven priors learned by a deep network specifically designed to imbibe weakly supervised constraints from the interplay of the unknown camera with 3D entities such as object heights, through estimation of bounding box projections. We leverage categorical priors for objects such as humans or cars that commonly occur in natural images, as references for scale estimation. We demonstrate state-of-the-art qualitative and quantitative results on several datasets as well as applications including virtual object insertion. Furthermore, the perceptual quality of our outputs is validated by a user study.

==> Sections/Figs/fig-allDataCOCOScale.tex <==
\begin{figure*}[!!t]
    \begin{center}
    % \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\scriptsize
% \begin{tabular}{Sc| Sc Sc Sc Sc}
% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{0.9\textwidth}{@{\hskip 0.15in}cccc@{}m{0pt}@{}}
% \begin{tabular*}{1\textwidth}{c |cc@{}m{0pt}@{}}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\

1 & 
\image{Figs/allDataCOCOScale/000001_393268_bboxes_merge_2_merge.png} &
\image{Figs/allDataCOCOScale/000002_262197_bboxes_merge_2_merge.png} &
\image{Figs/allDataCOCOScale/000003_393271_bboxes_merge_5_merge.png} \\ 
2 & 
\image{Figs/allDataCOCOScale/000009_000074_bboxes_merge_4_merge.png} &
\image{Figs/allDataCOCOScale/000013_000077_bboxes_merge_2_merge.png} &
\image{Figs/allDataCOCOScale/000016_262229_bboxes_merge_3_merge.png} \\ 
3 & 
\image{Figs/allDataCOCOScale/000023_262242_bboxes_merge_3_merge.png} &
\image{Figs/allDataCOCOScale/000024_131172_bboxes_merge_5_merge.png} &
\image{Figs/allDataCOCOScale/000025_393317_bboxes_merge_2_merge.png} \\ 
4 & 
\image{Figs/allDataCOCOScale/000029_524401_bboxes_merge_2_merge.png} &
\image{Figs/allDataCOCOScale/000038_524420_bboxes_merge_6_merge.png} &
\image{Figs/allDataCOCOScale/000043_262286_bboxes_merge_4_merge.png} \\ 
5 & 
\image{Figs/allDataCOCOScale/000053_524450_bboxes_merge_3_merge.png} &
\image{Figs/allDataCOCOScale/000056_393384_bboxes_merge_4_merge.png} &
\image{Figs/allDataCOCOScale/000074_131280_bboxes_merge_7_merge.png} \\ 

%  \hline 
% \bottomrule
\end{tabular*}

\end{center}
\vspace{-0.7cm}
% \captionsetup{labelformat=empty}
\caption{Examples of COCO-Scale-person. Each bounding box is a valid person acquired from our pruning.}
\label{fig:example_allDataCOCOScale}
\end{figure*}

==> Sections/Figs/fig-allDataKITTI.tex <==
\begin{figure*}[t!!]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1\textwidth}[t]{ccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\imageT{Figs/allDataKITTI/000001_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000002_kitti_reproj.jpg} \\ 
2 & 
\imageT{Figs/allDataKITTI/000003_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000004_kitti_reproj.jpg} \\ 
3 & 
\imageT{Figs/allDataKITTI/000005_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000006_kitti_reproj.jpg} \\ 
4 & 
\imageT{Figs/allDataKITTI/000007_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000008_kitti_reproj.jpg} \\ 
5 & 
\imageT{Figs/allDataKITTI/000009_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000010_kitti_reproj.jpg} \\ 
6 & 
\imageT{Figs/allDataKITTI/000011_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000012_kitti_reproj.jpg} \\ 
7 & 
\imageT{Figs/allDataKITTI/000013_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000014_kitti_reproj.jpg} \\ 
8 & 
\imageT{Figs/allDataKITTI/000015_kitti_reproj.jpg} &
\imageT{Figs/allDataKITTI/000016_kitti_reproj.jpg} \\ 


%  \hline 
% \bottomrule
\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{Examples of KITTI. Each bounding box is a valid object acquired from our pruning (pedestrians in green and cars in magenta).}
\label{fig:example_allDataKITTI}
\end{figure*}

==> Sections/Figs/fig-allIMDB_better.tex <==
%\vspace{-0.7cm}
\begin{figure*}[!!t]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1.\textwidth}[t]{cccccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\imageF{Supps/Figs/IMDB/better/000075_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/better/000075_M2-1_noKps_reproj.jpg} &
2 & 
\imageF{Supps/Figs/IMDB/better/000123_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/better/000123_M2-1_noKps_reproj.jpg}\\
3 & 
\imageF{Supps/Figs/IMDB/better/000132_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/better/000132_M2-1_noKps_reproj.jpg} &
4 & 
\imageF{Supps/Figs/IMDB/better/000774_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/better/000774_M2-1_noKps_reproj.jpg}\\

\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{Comparison between SN-L3-kps-can which incorporates keypoint estimation and upright ratio estimation (left), and SN-L3 which does not (right).}
\label{fig:more_IMDB_better}
\end{figure*}

% \vspace{-0.7cm}

==> Sections/Figs/fig-allIMDB_more.tex <==
%\vspace{-0.7cm}
\begin{figure*}[!!t]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1.\textwidth}[t]{ccccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\imageF{Supps/Figs/IMDB/more/000031_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000033_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000043_M1_reproj.jpg} & 
\imageF{Supps/Figs/IMDB/more/000044_M1_reproj.jpg}\\
2 & 
\imageF{Supps/Figs/IMDB/more/000045_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000046_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000047_M1_reproj.jpg} & 
\imageF{Supps/Figs/IMDB/more/000048_M1_reproj.jpg}\\
3 & 
\imageF{Supps/Figs/IMDB/more/000050_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000051_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000052_M1_reproj.jpg} & 
\imageF{Supps/Figs/IMDB/more/000053_M1_reproj.jpg}\\
4 & 
\imageF{Supps/Figs/IMDB/more/000054_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000055_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000057_M1_reproj.jpg} & 
\imageF{Supps/Figs/IMDB/more/000058_M1_reproj.jpg}\\
5 & 
\imageF{Supps/Figs/IMDB/more/000062_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000064_M1_reproj.jpg} &
\imageF{Supps/Figs/IMDB/more/000067_M1_reproj.jpg} & 
\imageF{Supps/Figs/IMDB/more/000068_M1_reproj.jpg}\\


% \addlinespace[0.05cm]

% \image{Figs/rendersRE/000119_M7_reproj.jpg} &
% \image{Figs/rendersRE/000119_M1_reproj.jpg} &
% \image{Figs/rendersRE/000119_M4_reproj.jpg} \\ 

% \addlinespace[0.05cm]


% \image{Figs/rendersRE/000081_M7_reproj.jpg} &
% \image{Figs/rendersRE/000081_M1_reproj.jpg} &
% \image{Figs/rendersRE/000081_M4_reproj.jpg} \\ 

% \addlinespace[0.05cm]


% \image{Figs/rendersRE/000080_M7_reproj.jpg} &
% \image{Figs/rendersRE/000080_M1_reproj.jpg} &
% \image{Figs/rendersRE/000080_M4_reproj.jpg} \\

% \addlinespace[0.05cm]


% \image{Figs/rendersRE/000066_M7_reproj.jpg} &
% \image{Figs/rendersRE/000066_M1_reproj.jpg} &
% \image{Figs/rendersRE/000066_M4_reproj.jpg} \\ 

% \addlinespace[0.05cm]

% \image{Figs/rendersRE/000022_M7_reproj.jpg} &
% \image{Figs/rendersRE/000022_M1_reproj.jpg} &
% \image{Figs/rendersRE/000022_M4_reproj.jpg} \\ 



%  \hline 
% \bottomrule
\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{More results of scene parameters estimation with SN-L3-kps-can on IMDB-23K. Person in red bounding box is the annotated person. The estimated height and ground truth height are labelled on the upper-left corner and over the bounding box respectively.}
\label{fig:more_IMDB_more}
\end{figure*}

% \vspace{-0.7cm}

==> Sections/Figs/fig-allKITTI2_better.tex <==
\begin{figure*}[t!!]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1\textwidth}[t]{ccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\imageT{Supps/Figs/KITTI/improve/000001_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000001_kitti_reproj.jpg} \\ 
2 & 
\imageT{Supps/Figs/KITTI/improve/000006_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000006_kitti_reproj.jpg} \\ 
3 & 
\imageT{Supps/Figs/KITTI/improve/000008_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000008_kitti_reproj.jpg} \\ 
4 & 
\imageT{Supps/Figs/KITTI/improve/000015_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000015_kitti_reproj.jpg} \\ 
5 & 
\imageT{Supps/Figs/KITTI/improve/000020_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000020_kitti_reproj.jpg} \\ 
6 & 
\imageT{Supps/Figs/KITTI/improve/000027_kitti_personInput_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000027_kitti_reproj.jpg} \\ 

\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{Comparison between SN-L3-mulCat with person only input (left), and SN-L3-mulCat with both person and car as input.}
\label{fig:more_KITTI_better}
% \vspace{-0.3cm}
\end{figure*}

% \vspace{-0.7cm}

==> Sections/Figs/fig-allKITTI2_more.tex <==
\begin{figure*}[t!!]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1\textwidth}[t]{ccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\

1 & 
\imageT{Supps/Figs/KITTI/more/000002_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000003_kitti_reproj.jpg} \\ 
2 & 
\imageT{Supps/Figs/KITTI/more/000005_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000008_kitti_reproj.jpg} \\ 
3 & 
\imageT{Supps/Figs/KITTI/more/000009_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000010_kitti_reproj.jpg} \\ 
4 & 
\imageT{Supps/Figs/KITTI/more/000009_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000012_kitti_reproj.jpg} \\ 
5 & 
\imageT{Supps/Figs/KITTI/more/000013_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000014_kitti_reproj.jpg} \\ 
6 & 
\imageT{Supps/Figs/KITTI/more/000015_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000016_kitti_reproj.jpg} \\ 
7 & 
\imageT{Supps/Figs/KITTI/more/000017_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000018_kitti_reproj.jpg} \\ 
8 & 
\imageT{Supps/Figs/KITTI/more/000019_kitti_reproj.jpg} &
\imageT{Supps/Figs/KITTI/more/000021_kitti_reproj.jpg} \\ 
% \imageT{Supps/Figs/KITTI/more/000022_kitti_reproj.jpg} &
% \imageT{Supps/Figs/KITTI/more/000023_kitti_reproj.jpg} \\ 

\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{More results of Scene parameters estimation with SN-L3-mulCat on KITTI-mulCat. Reprojected pedestrians are in blue, while cars are in magenta.}
\label{fig:more_KITTI_more}
% \vspace{-0.3cm}
\end{figure*}

% \vspace{-0.7cm}

==> Sections/Figs/fig-allReal.tex <==
\begin{figure*}[t!!]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1\textwidth}[t]{cc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\

\imageT{Figs/real/real-1.jpg_reproj.jpg} &
\imageT{Figs/real/real-8.jpg_reproj.jpg} \\ 

\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{Demo of two real-world samples where virtual object insertion is performed with our method.}
\label{fig:real_cases}
% \vspace{-0.3cm}
\end{figure*}

% \vspace{-0.7cm}

==> Sections/Figs/fig-allRenders2_better.tex <==
\begin{figure*}[t!!]
    \begin{center}
    \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\small
% \begin{tabular}{Sc| Sc Sc Sc Sc}
{\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{1\textwidth}[t]{ccccc@{}m{0pt}@{}}
% \begin{tabular}[t]{cccc}
% \toprule
% PGM & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\imageF{Supps/Figs/rendersRE2/corner/000003_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000003_M7_reproj.jpg} & 
\imageF{Supps/Figs/rendersRE2/corner/000090_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000090_M7_reproj.jpg} \\ 
2 & 
\imageF{Supps/Figs/rendersRE2/corner/000113_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000113_M7_reproj.jpg} & 
\imageF{Supps/Figs/rendersRE2/corner/000160_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000160_M7_reproj.jpg} \\ 

3 & 
\imageF{Supps/Figs/rendersRE2/corner/000013_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000013_M7_reproj.jpg} & 
\imageF{Supps/Figs/rendersRE2/corner/000087_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000087_M7_reproj.jpg} \\ 

4 & 
\imageF{Supps/Figs/rendersRE2/corner/000017_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000017_M7_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000107_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000107_M7_reproj.jpg} \\
5 & 
\imageF{Supps/Figs/rendersRE2/corner/000112_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000112_M7_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000133_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000133_M7_reproj.jpg} \\

6 & 
\imageF{Supps/Figs/rendersRE2/corner/000134_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000134_M7_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000155_M1_reproj.jpg} &
\imageF{Supps/Figs/rendersRE2/corner/000155_M7_reproj.jpg} \\

\end{tabular*}
}
\end{center}
% \captionsetup{labelformat=empty}
\vspace{-0.7cm}
\caption{Comparison on corner cases between SN-L3-mulCat (left in each pair), and PGM (right in each pair) on COCO-Scale-mulCat.}
\label{fig:more_coco_corner}
% \vspace{-0.3cm}
\end{figure*}

==> Sections/Figs/fig-allRenders2_fail.tex <==
\begin{figure*}[!!t]
    \begin{center}
    % \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\scriptsize
% \begin{tabular}{Sc| Sc Sc Sc Sc}
% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{0.9\textwidth}{@{\hskip 0.15in}cccccc@{}m{0pt}@{}}

1 & 
\image{Supps/Figs/rendersRE2/fail/000060_M1_reproj.jpg} &
2 & 
\image{Supps/Figs/rendersRE2/fail/000079_M1_reproj.jpg} &
3 & 
\image{Supps/Figs/rendersRE2/fail/000239_M1_reproj.jpg} \\ 

4 & 
\image{Supps/Figs/rendersRE2/fail/000099_M1_reproj.jpg} &
5 & 
\image{Supps/Figs/rendersRE2/fail/000109_M1_reproj.jpg} &
6 & 
\image{Supps/Figs/rendersRE2/fail/000194_M1_reproj.jpg} \\ 
% \bottomrule
\end{tabular*}

\end{center}
\vspace{-0.7cm}
% \captionsetup{labelformat=empty}
\caption{Failure cases results of scene parameters estimation and virtual object insertion on COCO-Scale with model COCO-Scale-mulCat.}
\label{fig:more_coco_fail}
% \vspace{-0.5cm}
\end{figure*}


==> Sections/Figs/fig-allRenders2_more.tex <==
\begin{figure*}[!!t]
    \begin{center}
    % \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\scriptsize
% \begin{tabular}{Sc| Sc Sc Sc Sc}
% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{0.9\textwidth}{@{\hskip 0.15in}cccc@{}m{0pt}@{}}
% \begin{tabular*}{1\textwidth}{c |cc@{}m{0pt}@{}}
% \toprule
% PGM* & SN-L3-kps-disc & SN-L1 \\ 
% M7 & M1 & M4\\
1 & 
\image{Supps/Figs/rendersRE2/more/000052_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000054_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000063_M1_reproj.jpg} \\ 
2 & 
\image{Supps/Figs/rendersRE2/more/000064_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000065_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000066_M1_reproj.jpg} \\ 
3 & 
\image{Supps/Figs/rendersRE2/more/000067_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000069_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000074_M1_reproj.jpg} \\ 
4 & 
\image{Supps/Figs/rendersRE2/more/000075_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000078_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000080_M1_reproj.jpg} \\

% \bottomrule
\end{tabular*}

\end{center}
\vspace{-0.7cm}
% \captionsetup{labelformat=empty}
\caption{More results of scene parameters estimation and virtual object insertion on COCO-Scale with model SN-L3-mulCat. The detected boxes are shown in green and reprojected ones in blue. The horizon is shown as a dashed blue line. Camera parameters are overlaid on the top. Chairs of 1m height are inserted alongside each person with the estimated parameters.}
\label{fig:more_coco_more}
% \vspace{-0.5cm}
\end{figure*}






\begin{figure*}[!!t]
    \begin{center}
    % \setlength{\tabcolsep}{0.05em}
    % \resizebox{1.\columnwidth}{!}{%
    % \setlength\extrarowheight{7pt}
%  trim={<left> <lower> <right> <upper>}

% \renewcommand{\arraystretch}{5}
% \begin{tabular}{Sc@{\hskip 0.04in}| Sc Sc Sc Sc@{\hskip 0.04in} @{}m{0pt}@{}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{Sc| Sc Sc Sc Sc@{}m{0pt}@{}}
\scriptsize
% \begin{tabular}{Sc| Sc Sc Sc Sc}
% {\renewcommand{\arraystretch}{1.2}% for the vertical padding
\begin{tabular*}{0.9\textwidth}{@{\hskip 0.15in}cccc@{}m{0pt}@{}}

1 & 
\image{Supps/Figs/rendersRE2/more/000081_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000082_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000083_M1_reproj.jpg} \\ 

2 & 
\image{Supps/Figs/rendersRE2/more/000089_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000096_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000105_M1_reproj.jpg} \\ 

3 & 
\image{Supps/Figs/rendersRE2/more/000112_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000118_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000122_M1_reproj.jpg} \\ 

4 & 
\image{Supps/Figs/rendersRE2/more/000123_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000126_M1_reproj.jpg} &
\image{Supps/Figs/rendersRE2/more/000135_M1_reproj.jpg} \\ 

% \bottomrule
\end{tabular*}

\end{center}
\vspace{-0.7cm}
% \captionsetup{labelformat=empty}
\caption{More results of scene parameters estimation and virtual object insertion on COCO-Scale with model SN-L3-mulCat (cont.)}
\label{fig:more_coco_more2}
% \vspace{-0.5cm}
\end{figure*}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
